Phenaki: Variable Length Video Generation From Open Domain Textual Description

We present Phenaki, a model capable of realistic video synthesis, given a sequence of textual prompts. Generating videos from text is particularly challenging due to the computational cost, limited quantities of high quality text-video data and variable length of videos. To address these issues, we introduce a new model for learning video representation which compresses the video to a small representation of discrete tokens. This tokenizer uses causal attention in time, which allows it to work with variable-length videos. To generate video tokens from text we are using a bidirectional masked transformer conditioned on pre-computed text tokens. The generated video tokens are subsequently de-tokenized to create the actual video. To address data issues, we demonstrate how joint training on a large corpus of image-text pairs as well as a smaller number of video-text examples can result in generalization beyond what is available in the video datasets. Compared to the previous video generation methods, Phenaki can generate arbitrary long videos conditioned on a sequence of prompts (i.e. time variable text or a story) in open domain. To the best of our knowledge, this is the first time a paper studies generating videos from time variable prompts. In addition, compared to the per-frame baselines, the proposed video encoder-decoder computes fewer tokens per video but results in better spatio-temporal consistency.

==> tables/t2v_comparison.tex <==
\begin{table}
\small
\caption{Text-to-video comparisons on Kinetics-400~\cite{Kinetics400}.}
\vspace{-.3cm}
\label{table:t2v_comp}
\begin{center}
\begin{tabular}{lrr}
Method  & FID-img $\downarrow$ & FID-vid $\downarrow$ \\
\hline
T2V \cite{vidgenfromtext}     & 82.13 & 14.65 \\
SC \cite{tfgan}                 & 33.51 & 7.34 \\
TFGAN \cite{tfgan}                   & 31.76 & 7.19 \\
NUWA                      & \textbf{28.46} & 7.05 \\
\hline
Phenaki [Zero Shot] (Ours)            & 37.74 & \textbf{3.84} \\
\end{tabular}
\end{center}
\end{table}

==> tables/t2v_results.tex <==
% \mbz{coming soon!}

\begin{table}
\small
\caption{Text-to-video and text-to-image results highlighting the importance of image datasets in video models. Text-to-image evaluation is done on $40960$ images in LAION-400M~\cite{schuhmann2021laion}.
%\rubville{cfg=6, temp=4, iterations=24, over 4096 videos from lms}
}
\vspace{-.3cm}
\label{tab:video_image}
\centering
\begin{tabular}{c|lll|ll}
Data Split & \multicolumn{3}{|c|}{Text to Video} & \multicolumn{2}{c}{Text to Image} \\\hline\hline
Videos\% / Images\% & CLIP $\uparrow$ & FID $\downarrow$ & FVD $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$ \\\hline
100\% / 0\% & 0.298 & \textbf{19.2} & \textbf{168.9} & 0.240 & 53.9\\
80\% / 20\% & \textbf{0.303} & 21.4 & 198.4 & \textbf{0.289} & \textbf{29.4}\\
50\% / 50\%& 0.302 & 21.4 & 239.7 & 0.287 & 30.5\\             
\end{tabular}

% \ Data Split  & Text2Video & Text2Image \\
% \begin{tabular}{cccccc}
% \ \ \ \ \ Videos\% / Images\%  & CLIP $\uparrow$ & FID $\downarrow$ & FVD $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$\\
% \hline
% 100\% / 0\%                    & 0.298 & 19.2 & \textbf{168.9} & - & -\\
% \ \ \ \ 80\% / 20\%            & \textbf{0.303} & 21.4 & 198.4 & - & -\\
% \ \ \ \ 50\% / 50\%            & 0.302 & 21.4 & 239.7 & - & -\\
% \end{tabular}
% \end{tabular}
\end{table}
